A Conforming Finite Element Discretization of the Streamfunction Form of the Unsteady Quasi-Geostrophic Equations

This paper presents a conforming finite element semi-discretization of the streamfunction form of the one-layer unsteady quasi-geostrophic equations, which are a commonly used model for large-scale wind-driven ocean circulation. We derive optimal error estimates and present numerical results.

==> makefile <==
LFLAGS=-halt-on-error -file-line-error
LDRAFTFLAGS=-draftmode $(LFLAGS)
UNAME = $(shell uname)
CWD = $(shell pwd)
# the command to create a temporary folder varies by platform.
ifeq ($(UNAME), Darwin)
	PDFLATEX = "/usr/local/texlive/2012/bin/x86_64-darwin/pdflatex"
	BIBTEX = "/usr/local/texlive/2012/bin/x86_64-darwin/bibtex"
	TMPCMD = $(shell TMPDIR=$(CWD) && mktemp -t TMPMAIN)
else
	PDFLATEX = $(shell which pdflatex)
	BIBTEX = $(shell which bibtex)
	TMPCMD = $(shell mktemp --tmpdir=$(CWD) -t XXXXXXXX)
endif

.PHONY: setuptemp

QGE.pdf: paper

# Check for errors; this is useful for setting up the temporary files because
# make will exit (without deleting temporaries) if compilation fails.
quickcheck: *.tex
	@$(PDFLATEX) $(LDRAFTFLAGS) QGE.tex | python filter.py

setuptemp: quickcheck
	@$(eval TMPMAINROOT = $(TMPCMD))
	@$(eval TMPMAINTEX = $(TMPMAINROOT).tex)
	@$(eval TMPMAINBASE = $(shell basename $(TMPMAINROOT)))

# 3/4 of the runs needed to compile.
first3: *.tex
	@$(PDFLATEX) $(LDRAFTFLAGS) QGE.tex | python filter.py
	@$(BIBTEX) QGE 1>/dev/null
	@$(PDFLATEX) $(LDRAFTFLAGS) QGE.tex 1>/dev/null

# Compile with no options.
paper: first3
	@$(PDFLATEX) $(LFLAGS) QGE.tex 1>/dev/null

# Compile with the nag package.
nag: *.tex setuptemp
	@printf "\\RequirePackage[l2tabu, orthodox]{nag}\n" >> $(TMPMAINTEX)
	@cat QGE.tex >> $(TMPMAINTEX)
	@$(PDFLATEX) $(LDRAFTFLAGS) $(TMPMAINTEX) 1>/dev/null
	@$(BIBTEX)   $(TMPMAINBASE) 1>/dev/null
	@$(PDFLATEX) $(LDRAFTFLAGS) $(TMPMAINTEX) 1>/dev/null
	@$(PDFLATEX) $(LFLAGS)    $(TMPMAINTEX) | python filterwarn.py
	@rm $(TMPMAINROOT)*

# Compile and show LaTeX warnings.
warn: first3
	@$(PDFLATEX) $(LFLAGS) QGE.tex | python filterwarn.py

# Compile with date of last commit.
withversion: *.tex setuptemp
	@cat QGE.tex | python addrevision.py > $(TMPMAINTEX)
	@$(PDFLATEX) $(LDRAFTFLAGS) $(TMPMAINTEX) 1>/dev/null
	@$(BIBTEX)   $(TMPMAINBASE) 1>/dev/null
	@$(PDFLATEX) $(LDRAFTFLAGS) $(TMPMAINTEX) 1>/dev/null
	@$(PDFLATEX) $(LFLAGS)      $(TMPMAINTEX) 1>/dev/null
	@mv $(TMPMAINBASE).pdf QGE.pdf
	@rm $(TMPMAINROOT)*

